QoS-aware User Grouping Strategy for Downlink Multi-Cell NOMA Systems

In multi-cell non-orthogonal multiple access (NOMA) systems, designing an appropriate user grouping strategy is an open problem due to diverse quality of service (QoS) requirements and inter-cell interference. In this paper, we exploit both game theory and graph theory to study QoS-aware user grouping strategies, aiming at minimizing power consumption in downlink multi-cell NOMA systems. Under different QoS requirements, we derive the optimal successive interference cancellation (SIC) decoding order with inter-cell interference, which is different from existing SIC decoding order of increasing channel gains, and obtain the corresponding power allocation strategy. Based on this, the exact potential game model of the user grouping strategies adopted by multiple cells is formulated. We prove that, in this game, the problem for each player to find a grouping strategy can be converted into the problem of searching for specific negative loops in the graph composed of users. Bellman-Ford algorithm is expanded to find these negative loops. Furthermore, we design a greedy based suboptimal strategy to approach the optimal solution with polynomial time. Extensive simulations confirm the effectiveness of grouping users with consideration of QoS and inter-cell interference, and show that the proposed strategies can considerably reduce total power consumption comparing with reference strategies.

==> README <==
README
------

  The subfigure package has been superseded by the subfig package.
  The reason for the name change is that the new subfig package is not
  exactly backward compatible with this package; although, it comes
  with a configuration file that *almost* allows backward
  compatibility, the difference is that exact spacing and layout of
  the subfloats are not preserved.

  The newer (subfig) package is an improvement over this package and
  although this package will continue to be supported, it will no longer
  be updated.

This directory contains version 2.1.5 of the subfigure package.
Use `make' to extract the subfigure package and run the local tests.

MANIFEST:
---------
Makefile           UNIX makefile to extract the subfigure package
                       and related material.
README             This file.
subfigure.dtx      The documented subfigure package.
subfigure.ins      The subfigure package installation file.
subfigure.pdf      Subfigure package documentation (as PDF).
test.tex           Test one: Mixed tables and figures.
test2.tex          Test two: Check for extra space around figure
test3.tex          Test four: Test of optional args and \subref.
test4.tex          Test four: Test of interaction with hyperref.
test5.tex          Test five: Test for class \let of \endfigure, etc.

FILES AFTER `make':
-------------------
Makefile           UNIX makefile to extract the subfigure package
                       and related material.
README             This file.
ltxdoc.cfg         Configuration file to print change history and
                       index on the subfigure package documentation.       
subfigure.cfg      Set the preferred options for subfigure version 2.1.
subfigure.dtx      The documented subfigure package.
subfigure.ins      The subfigure package installation file.
subfigure.pdf      Subfigure package documentation (as PDF).
subfigure.ps       Subfigure package documentation (as PostScript).
subfigure.sty      The subfigure package 
test.ps            Results of test one.
test.tex           Test one: Mixed tables and figures.
test2.ps           Results of test two.
test2.tex          Test two: Check for extra space around figure
test3.ps           Results of test three.
test3.tex          Test four: Test of optional args and \subref.
test4.pdf          Results of test four.
test4.tex          Test four: Test of interaction with hyperref.
test5.tex          Test five: Test for class \let of \endfigure, etc.
test5a.ps          Results of test five (log file).
test5b.ps          Results of test five (output).

NOTES:
------

By default, the subfigure.sty file acts like the older versions of the
subfigure package.  To make the preferred options default move the
subfigure.cfg file into the standard TEXINPUTS path along with the
subfigure.sty file.  This reduces the whitespace around the subfigures
and subtables and sets the table style to have the captions and
subcaptions preceed the table and subtables.

